Clinical Concept Extraction for Document-Level Coding

The text of clinical notes can be a valuable source of patient information and clinical assessments. Historically, the primary approach for exploiting clinical notes has been information extraction: linking spans of text to concepts in a detailed domain ontology. However, recent work has demonstrated the potential of supervised machine learning to extract document-level codes directly from the raw text of clinical notes. We propose to bridge the gap between the two approaches with two novel syntheses: (1) treating extracted concepts as features, which are used to supplement or replace the text of the note; (2) treating extracted concepts as labels, which are used to learn a better representation of the text. Unfortunately, the resulting concepts do not yield performance gains on the document-level clinical coding task. We explore possible explanations and future research directions.

==> old/quant_experiments.tex <==
\subsection{Datasets}
\input{tables/datasets}
\input{tables/concept_extr_stats}

The MIMIC-III dataset is a collection of deidentified discharge summaries collected from ICU patient stays at the Beth Israel Deaconess Medical Center between 2001 and 2012 (\todo{cite}). Each discharge summary has been tagged with a set of ICD codes (\todo{cite}) representing the diagnoses and procedures which occurred during that visit. These are labeled by a human coder from a set of about 13,000 possible (diagnosis) codes. Many codes can be assigned to a visit in conjunction with one another.

The Sutter CHF cohort consists of progress notes for patient hospital visits from ten years prior to a heart failure diagnosis up to the diagnosis itself (or ten years from the last progress note date, for a control patient). \note{current file includes all visits right up to the index date. Consider predicting early-onset instead} 

See Table \ref{tab:stats} for descriptive statistics on the three datasets used in our experiments, and Table \ref{tab:CE} for statistics on the results of performing pre-modeling concept extraction on them. We selected datasets of varying size, patient distribution, and text length, and with different label sets for prediction, in order to test \name{} in different settings.

\paragraph{Preprocessing}
For the MIMIC-III dataset, we follow the same procedure outlined in CAML, specifically to "remove tokens that contain no alphabetic characters, lowercase all tokens, and replace tokens that appear in fewer than three training documents with an `UNK' token...truncat[ing all documents] to a maximum length of 2500 tokens." We concatenate all supplemental text for a patient discharge summary into one record, following the data processing pipeline provided by the authors of CAML\footnote[1]{\url{https://github.com/jamesmullenbach/caml-mimic/blob/master/notebooks/dataproc_mimic_III.ipynb}}. We refer the reader to that paper for further details.

For the Sutter CHF cohort, we follow the same procedure. \todo{get distribution of text length for establishing cutoff point- for reference, the min. text length is 1 word but max. is 19,438. 75th percentile is 440 words. Likely removing outliers may be better than just chopping at 2,500.} Note: we initially considered concatenating all patient text into one record, but this holds a potential disadvantage of diluting the attention distribution over the text, since we would then be convolving and attending over sequences of 20-30,000 tokens.

We also ensure for all cohorts (but particularly relevant for the Sutter HF one) that all notes for a single patient are assigned to either the test, training, or development set, so that there is no patient overlap, which could unfairly advantage the model.

\subsection{Concept Extraction} \label{CE}

We build a custom dictionary from the UMLS Metathesaurus \todo{cite} that includes ICD9CM, ICD10CM, ICD10PCS, RXNORM and SNOMEDCT\_US mappings, and ran the cTAKES annotator in advance of training for all 3 dataset splits using the resulting dictionary. Statistics on the number of extracted concepts per concept type and note can be found in Table \ref{tab:CE}. Details on the size of the concept vocabulary can be found in Table \ref{tab:model-details}. We also augment our concept vocabulary to include the (unobserved) CCS codes up the hierarchy \todo{any other hierarchical ontologies?}, and include them during our concept embedding initialization scheme described in Section \ref{concept_embeds}.

\subsection{Baselines} \label{baseline}
We utilize the open-source implementation of CAML\footnote[2]{\url{https://github.com/jamesmullenbach/caml-mimic}} as a baseline, adjusting it to a binary classification setting in the heart failure prediction case. 

We also run and report results for baseline models which leverage the extracted concept embeddings, but do not learn their representations with a GRAM-style methodology, instead just using their individual embeddings to represent themselves. We also group the ICD9 extracted concepts into the different levels of specificity present in the CCS grouper, since prior work has shown that grouping codes improves performance \todo{cite Robert's paper here}, in order to see if reducing the parameter space size and allowing for more observations of the concepts during training can improve the overall performance of the model, as well as if attending over the CCS hierarchy tree is necessary. Diagnosis codes are grouped into up to 4 CCS groups of less and less specificity, while procedures are grouped into up to 3. We test all of these as input representations of the concepts. \todo{move this paragraph to methods?}

\todo{other baselines: Random DAG, concept embeddings but no GRAM tree, \textit{just using the extracted concepts as inputs themselves sans text}, \textit{just using the extracted ICD concepts as the prediction directly}, etc.}

We also consider a baseline of using just the extracted concepts as input, instead of the concept-augmented text, or appended to the standard text. In the heart-failure prediction case... Note this baseline would not be able to provide natural-language explanations.

\note{None of the baselines have been run yet- holding off until more validation of core method value first}

\subsection{Implementation}

All neural models are implemented using PyTorch\footnote[3]{\url{https://github.com/pytorch/pytorch}}. We use the same early stopping criteria of 10 epochs on the precision at 8 criterion as in the original CAML paper, and port the optimal hyperparameters from CAML to \name{} as well. See Table \ref{tab:model-details} for model specifics.

For the word-concept-pairs interpolation method described in Section \ref{input-rep}, we use all word-concept occurrences for which there are at least two examples in the training set to define the matrix. We also initialize interpolation constants for the following additional cases: (UNK word, known concept), (known word, UNK concept), and a general UNK token, if both the word and concept terms are unknown in their respective vocabularies and/or during test-time if the word-concept pair has not been observed in the training set. 

Annotating the MIMIC datafiles using the specifications listed in Section \ref{CE} takes between 4 and 5 hours for 3,000 discharge summaries in the MIMIC dataset on a single CPU. This process can be parallelized for efficiency.

\name{} takes approximately 15 hours to train (compared to 8 hours for CAML) on a single NVIDIA Titan X GPU with 12189 MiB of RAM. For computational efficiency, we don't prune tree size before computing attention over parents for batch. This results in some attention being given to pad vectors, but manual inspection shows this attention score to generally be lower than the true embeddings of the tree, so we select to make this tradeoff.
\note{I don't think GRAM was done in this way, but I don't think it's feasible in this setting to sub-group each batch for that calculation considering we are already batching on text length. Initially tried this way and time to train was infeasibly longer.} \todo{Discussed with Edward and need to reformat the tree size, will lengthen training time by some factor}

\subsection{Parameter tuning}
\todo{tune the hyperparameters of \name{} using the Spearmint Bayesian optimization package \cite{NIPS2012_4522, NIPS2013_5086}.\footnote[4]{\url{https://github.com/HIPS/Spearmint}}}

%\input{tables/hyperparams.tex}
\input{tables/model_details.tex}

\subsection{Evaluation Metrics} 

==> scripts/abstract.tex <==
% Hard to follow the flow of the argument; when you feel like your abstract needs more than one paragraph, that's a sign that something has gone wrong. -J
Large patient records generated by the electronic health records (EHR) system have led to recent studies showing improved predictive healthcare based on advanced computational methods. 
%Although many studies focus on the structured part of the EHR such as diagnosis codes and lab measures, 
Recent work has shown impressive results using deep learning models based fully on raw-text clinical notes, where detailed patient information and clinical assessments lie. 

Clinical information extraction tools have long served as a means for automatically extracting structured data from the text of a patient record, and provide a source of cultivated domain knowledge. However, it is still an unanswered question how helpful the information provided by such tools can be in prediction tasks based on clinical text.
%How helpful can this information be, and how best to incorporate it, in prediction tasks on clinical text using new, advanced deep learning models?
We experiment with Apache clinical Text Analysis Knowledge Extraction System (cTAKES), the most widely used clinical information extraction tool, and present two architectures for leveraging cTAKES' annotations to mitigate the shortcomings of raw-text models. We highlight cTAKES' shortcomings in producing performance gains on the clinical coding task, and suggest directions for future work. 

==> tables/aux_task_aux_results_old.tex <==
\begin{table}[ht]
\centering
\resizebox{\columnwidth}{!}{\begin{tabular}{l|l|l|l|l}
\toprule
\textbf{Shared Features} & \textbf{Auxiliary Model} & \lambda & \multicolumn{2}{c}{\textbf{Tagging Accuracy}}\\ 
&  & & \textbf{After one epoch} &  \textbf{After last epoch}\\ 
\midrule
Pre-convolution & MLP & 0.0001 & 0.915 & 0.936 \\
Pre-convolution & MLP & 0.1 & 0.922 & 0.938 \\
Pre-convolution & MLP & 1.0 & 0.922 & 0.938 \\
Pre-convolution & MLP & 1000 & 0.922 & 0.938 \\
Pre-convolution & Linear Layer & 1.0 & 0.827 & 0.937 \\
Post-convolution & MLP & 1.0 & 0.797 & 0.929 \\
Post-convolution & Linear Layer & 1.0 & 0.526 & 0.929 \\
\bottomrule
\end{tabular}}
\caption{The effect of tuning $\lambda$ on dev set performance on the auxiliary task. Note that the high task performance is achieved even after one epoch with a simple model. \todo{reference somewhere in text}}
\label{tab:aux_aux}
\end{table}
